Look Before You Leap: An Exploratory Study of Uncertainty Measurement for Large Language Models

The recent performance leap of Large Language Models (LLMs) opens up new opportunities across numerous industrial applications and domains. However, erroneous generations, such as false predictions, misinformation, and hallucination made by LLMs, have also raised severe concerns for the trustworthiness of LLMs', especially in safety-, security- and reliability-sensitive scenarios, potentially hindering real-world adoptions. While uncertainty estimation has shown its potential for interpreting the prediction risks made by general machine learning (ML) models, little is known about whether and to what extent it can help explore an LLM's capabilities and counteract its undesired behavior. To bridge the gap, in this paper, we initiate an exploratory study on the risk assessment of LLMs from the lens of uncertainty. In particular, we experiment with twelve uncertainty estimation methods and four LLMs on four prominent natural language processing (NLP) tasks to investigate to what extent uncertainty estimation techniques could help characterize the prediction risks of LLMs. Our findings validate the effectiveness of uncertainty estimation for revealing LLMs' uncertain/non-factual predictions. In addition to general NLP tasks, we extensively conduct experiments with four LLMs for code generation on two datasets. We find that uncertainty estimation can potentially uncover buggy programs generated by LLMs. Insights from our study shed light on future design and development for reliable LLMs, facilitating further research toward enhancing the trustworthiness of LLMs.

==> table/code_discussion.tex <==


\begin{table*}[htbp]
    \caption{The average distances between code generated by open- and closed-source LLMs.}
    \centering
    \responseref{}
    \renewcommand{\arraystretch}{1.1}
    \footnotesize
    \label{tab:code_sutble}
    % \resizebox{0.85\columnwidth}{!}{
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}{lccccccccc}
    \toprule
    & \multicolumn{2}{c}{\textbf{HumanEval}} &&  \multicolumn{2}{c}{\textbf{MBPP}}  \\
    \cmidrule{2-5} \cmidrule{5-8}
    & Codegen & Incoder  & Santacoder & Code Llama &&  Codegen & Incoder  & Santacoder & Code Llama \\
    \midrule
    Cosine & 0.03$\pm$0.04 & 0.03$\pm$0.05  && 0.03$\pm$0.02 & 0.02$\pm$0.01 \\
    %Cosine & 0.03$\pm$0.02 & 0.03$\pm$0.02  && 0.03$\pm$0.03 & 0.01$\pm$0.01 \\
    CodeBLEU & 0.53$\pm$0.19 & 0.45$\pm$0.19  && 0.71$\pm$0.10 & 0.41$\pm$0.16 \\
    \bottomrule
    \end{tabular}
    \vspace{-10pt}
    % }
    % \vspace{-1mm}
\end{table*}

==> table/code_pass.tex <==


\begin{table}[!tb]
    \caption{\textit{Pass@1} rate of different LLMs.}
    \centering
    \small
    \label{tab:code_bench}
     % \resizebox{0.75\columnwidth}{!}{
    \begin{tabular}{lll}
    \toprule
    & \textbf{Humaneval} & \textbf{MBPP} \\
    \midrule
    Incoder & 14.6\% (24/164) & 16.6\% (83/500) \\
    SantaCoder & 1.2\% (2/164) & 8.8\% (44/500) \\
    CodeGen & 21.3\% (35/164) & 28.6\% (143/500) \\
    \cellcolor{lightgray}GPT3.5 & \cellcolor{lightgray}80.0\% (32/40) & \cellcolor{lightgray}58.4\% (73/125) \\
    \bottomrule
    \end{tabular}
    \vspace{-10pt}
     % }
\end{table}

==> table/code_performance_old.tex <==
\begin{table*}[htbp]
  \centering
  %\responseref{}
  %Pearson correlation coefficients between uncertainty scores and LLMs' performance on two code generation tasks.
  \caption{AUC scores for detecting erroneous code generated by LLMs. The results of VR/VRO are presented as ``{\em cosine distance-based (task-specific distance-based)}.'' Highest scores are ranked and highlighted as \colorbox{top1Color}{\textit{top-1}}, \colorbox{top2Color}{\textit{top-2}}, and \colorbox{top3Color}{\textit{top-3}}.}
  % \vspace{-2mm}
  \renewcommand{\arraystretch}{1.1}
  \label{tab:evaluation_corrCode}
  \begin{subtable}[h]{\textwidth}
    \setlength{\tabcolsep}{10pt}
    \centering
\responseref{}

    % \caption{Single-inference/Sample-based Uncertainty Estimation}
    \scriptsize
        % \resizebox{0.95\linewidth}{!}{
        \begin{tabular}{llccccccccc}
        \toprule
        % \rotatebox[origin=c]{90}{rota}}
        \multirow{2}{*}{\textbf{Dataset}}&\multirow{2}{*}{\textbf{LLM}} & \multicolumn{4}{c}{{\bf Single-inference Method}} && \multicolumn{2}{c}{{\bf Sample-based Method}}\\
        \cmidrule{3-6} \cmidrule{8-9}
        && \textbf{Max Prob} & \textbf{Average Prob} & \textbf{Max Ent} & \textbf{Average Ent} && \textbf{Sample VR} & \textbf{Sample VRO}\\
        \cmidrule{1-6} \cmidrule{8-9}
        \multirow{7}{*}{{HumanEval}} & CodeQwen1.5 &0.592 & 0.539 & 0.578 & 0.538 && 0.639(0.617) & \toponehl{0.668}(\toptwohl{0.647})  \\

        & DeepSeek Coder & \topthreehl{0.735} & 0.692 & \toptwohl{0.738} & 0.676 && 0.730(0.705) & \toponehl{0.747}(0.699)  \\

        & Starcoder2 & \topthreehl{0.747} & 0.629 & \toponehl{0.752} & 0.656 && 0.693(0.675) & \toptwohl{0.748}(0.670)  \\

        & Code Llama& \topthreehl{0.744} & 0.618 & \toponehl{0.752} & 0.601 && 0.697(0.681) & 0.731(\toptwohl{0.749})\\


        & GPT3.5 & 0.500 & 0.590 & 0.383 & 0.490 && 0.630(\toponehl{0.667}) & \toptwohl{0.607}(0.587) \\

        & GPT4o mini & \toponehl{0.909} & \topthreehl{0.760} & \toptwohl{0.891} & 0.749 && 0.657(0.583) & 0.737(0.714) \\

        & GPT4o & 0.583 & 0.623 & 0.480 & 0.543 && 0.423(0.623) & 0.343(0.606) \\


        \cellcolor{lightgray}& \cellcolor{lightgray}CodeQwen1.5 & \cellcolor{lightgray}0.356 & \cellcolor{lightgray}0.363 & \cellcolor{lightgray}0.358 & \cellcolor{lightgray}0.367 && \cellcolor{lightgray}0.555(\toptwohl{0.613}) & \cellcolor{lightgray}\topthreehl{0.593}(\toponehl{0.643})   \\
        
        \cellcolor{lightgray}& \cellcolor{lightgray}DeepSeek Coder & \cellcolor{lightgray}0.545 & \cellcolor{lightgray}0.463 & \cellcolor{lightgray}0.527 & \cellcolor{lightgray}0.46 && \cellcolor{lightgray}0.581({0.618}) & \cellcolor{lightgray}0.617(\topthreehl{0.621})	  \\
        


        \cellcolor{lightgray}& \cellcolor{lightgray}Starcoder2 & \cellcolor{lightgray} 0.567 & \cellcolor{lightgray} 0.447 & \cellcolor{lightgray} 0.589 & \cellcolor{lightgray} 0.439 && \cellcolor{lightgray} 0.562(0.616) & \cellcolor{lightgray} 0.581(\toponehl{0.665})  \\

        \cellcolor{lightgray}& \cellcolor{lightgray}Code Llama & \cellcolor{lightgray}0.499 & \cellcolor{lightgray}0.418 & \cellcolor{lightgray}0.483 & \cellcolor{lightgray}0.433 && \cellcolor{lightgray}0.578(\topthreehl{0.668}) & \cellcolor{lightgray}0.603(\toponehl{0.705})\\

        \cellcolor{lightgray} & \cellcolor{lightgray}GPT3.5 & \cellcolor{lightgray}\topthreehl{0.582} & \cellcolor{lightgray}0.556 & \cellcolor{lightgray}\toptwohl{0.606} & \cellcolor{lightgray}0.560 && \cellcolor{lightgray}0.592(0.563) & \cellcolor{lightgray}0.561(0.576)  \\


         \cellcolor{lightgray}& \cellcolor{lightgray}GPT4o mini & \cellcolor{lightgray} 0.579 & \cellcolor{lightgray} 0.609 & \cellcolor{lightgray} 0.593 & \cellcolor{lightgray} \topthreehl{0.628} && \cellcolor{lightgray} 0.609(0.606) & \cellcolor{lightgray} 0.599(0.569)  \\

        \multirow{-7}{*}{\cellcolor{lightgray}{MBPP}} & \cellcolor{lightgray}GPT4o & \cellcolor{lightgray} 0.629 & \cellcolor{lightgray} 0.633 & \cellcolor{lightgray} 0.635 & \cellcolor{lightgray} \topthreehl{0.667} && \cellcolor{lightgray} 0.650(\toponehl{0.735}) & \cellcolor{lightgray} 0.634(\toptwohl{0.698})  \\

        \bottomrule
        \end{tabular}
        % }
  \end{subtable}
  \vspace{6pt}
  \vfill
  \begin{subtable}[h]{\textwidth}
  \setlength{\tabcolsep}{9.98pt}
  \centering
\responseref{}

  % \caption{Perturbation-based Uncertainty Estimation}
  \scriptsize
  % \resizebox{0.95\linewidth}{!}{
    \begin{tabular}{llcccccc}
        \toprule
        \multirow{2}{*}{\textbf{Dataset}}&\multirow{2}{*}{\textbf{LLM}} & \multicolumn{6}{c}{\textbf{Perturbation-based}}\\
        \cmidrule{3-8}
        && \textbf{Max VR} & \textbf{Max VRO} & \textbf{Min VR} & \textbf{Min VRO} & \textbf{MaxDiff VR} & \textbf{MaxDiff VRO} \\
        \midrule
        
        \multirow{7}{*}{HumanEval} & CodeQwen1.5 & 0.629(0.611) & \topthreehl{0.646}(0.609) & 0.595(0.592) & 0.593(0.571) & 0.626(0.627) & 0.638(0.595)
         \\
   
        
        & DeepSeek Coder & 0.607(0.479) & 0.664(0.512) & 0.589(0.563) & 0.574(0.426) & 0.604(0.454) & 0.661(0.581)	  \\

         & Starcoder2 & 0.638(0.569) & 0.664(0.643) & 0.449(0.457) & 0.565(0.526) & 0.592(0.525) & 0.666(0.629) \\

         & Code Llama & 0.597(0.613) & 0.668(0.644) & 0.498(0.555) & 0.643(0.582) & 0.609(0.538) & 0.725(0.680)  \\

        & GPT3.5 & 0.500(0.503) & 0.457(0.560) & 0.497(0.503) & 0.420(\topthreehl{0.607}) & 0.533(0.533) & 0.393(0.477)  \\

        & GPT4o mini & 0.546(0.531) & 0.703(0.743) & 0.594(0.531) & 0.589(0.646) & 0.506(0.460) & 0.686(0.749)  \\

        & GPT4o & 0.571(0.560) & \toptwohl{0.709}(\toponehl{0.720}) & 0.391(0.469) & 0.600(0.674) & 0.457(0.509) & \topthreehl{0.691}(0.680) \\

        \cellcolor{lightgray} & \cellcolor{lightgray}CodeQwen1.5 & \cellcolor{lightgray}0.533(0.532) & \cellcolor{lightgray}0.501(0.553) & \cellcolor{lightgray}0.476(0.478) & \cellcolor{lightgray}0.487(0.520) & \cellcolor{lightgray}0.567(0.553) & \cellcolor{lightgray}0.523(0.558) \\

        \cellcolor{lightgray} & \cellcolor{lightgray}DeepSeek Coder & \cellcolor{lightgray}0.620(0.592) & \cellcolor{lightgray}0.561(0.566) & \cellcolor{lightgray}0.456(0.480) & \cellcolor{lightgray}0.459(0.487) & \cellcolor{lightgray}\toponehl{0.658}(\toptwohl{0.654}) & \cellcolor{lightgray}0.619(0.619)  \\


        \cellcolor{lightgray} & \cellcolor{lightgray}Starcoder2 & \cellcolor{lightgray} 0.600(0.576) & \cellcolor{lightgray} 0.568(0.587) & \cellcolor{lightgray} 0.485(0.451) & \cellcolor{lightgray} 0.420(0.477) & \cellcolor{lightgray} \toptwohl{0.635}(\topthreehl{0.632}) & \cellcolor{lightgray} 0.570(0.627) \\

        \cellcolor{lightgray} & \cellcolor{lightgray}Code Llama & \cellcolor{lightgray}0.586(0.630) & \cellcolor{lightgray}0.521(0.621) & \cellcolor{lightgray}0.454(0.507) & \cellcolor{lightgray}0.501(0.568) & \cellcolor{lightgray}0.622(\toptwohl{0.679}) & \cellcolor{lightgray}0.566(0.667)	 \\
        
        \cellcolor{lightgray} & \cellcolor{lightgray}GPT3.5 & \cellcolor{lightgray}0.587(\toponehl{0.628}) & \cellcolor{lightgray}0.511(0.544) & \cellcolor{lightgray}0.550(0.495) & \cellcolor{lightgray}0.508(0.511) & \cellcolor{lightgray}0.498(0.571) & \cellcolor{lightgray}0.486(0.528)  \\
        

        \cellcolor{lightgray} & \cellcolor{lightgray}GPT4o mini & \cellcolor{lightgray} 0.574(0.487) & \cellcolor{lightgray} 0.574(0.463) & \cellcolor{lightgray} 0.416(0.397) & \cellcolor{lightgray} 0.420(0.435) & \cellcolor{lightgray} \toptwohl{0.650}(0.551) & \cellcolor{lightgray} \toponehl{0.675}(0.533)	 \\
        
        
        \multirow{-7}{*}{\cellcolor{lightgray}MBPP} & \cellcolor{lightgray}GPT4o & \cellcolor{lightgray}0.448(0.538) & \cellcolor{lightgray}0.418(0.546) & \cellcolor{lightgray}0.560(0.591) & \cellcolor{lightgray}0.536(0.549) & \cellcolor{lightgray}0.514(0.545) & \cellcolor{lightgray}0.454(0.495)	 \\
        
        \bottomrule
    \end{tabular}
    % }
    \end{subtable}
    % \vspace{-2mm}
\end{table*}

==> table/nlp_performance_old.tex <==
% OLD Table V2
\iffalse
\begin{table*}[htbp]
  \centering
  \caption{Pearson correlation coefficients between uncertainty scores and LLMs' performance on four NLP tasks. The results of VR/VRO are presented as ``{\em cosine distance-based (task-specific distance-based)}.'' Highest correlations from different categories are ranked and highlighted as \colorbox{top1Color}{\textit{top-1}}, \colorbox{top2Color}{\textit{top-2}}, and \colorbox{top3Color}{\textit{top-3}}. 
  %\jiayang{I altered the color for \emph{top-1}, it was kind of overshadowing}
  }
  \renewcommand{\arraystretch}{1.1}
  \begin{subtable}[h]{\textwidth}
    \setlength{\tabcolsep}{11pt}
    \centering
    %\responseref{}
    % \caption{Single-inference/Sample-based Uncertainty Estimation}
    \scriptsize
        \resizebox{0.95\linewidth}{!}{
        \begin{tabular}{llcccccll}
        \toprule
        % \rotatebox[origin=c]{90}{rota}}
        \multirow{2}{*}{\textbf{Dataset}}&\multirow{2}{*}{\textbf{LLM}} & \multicolumn{4}{c}{{\bf Single-inference Method}} && \multicolumn{2}{c}{{\bf Sample-based Method}}\\
        \cmidrule{3-6} \cmidrule{8-9}
        && \textbf{Max Prob} & \textbf{Average Prob} & \textbf{Max Ent} & \textbf{Average Ent} && \textbf{Sample VR} & \textbf{Sample VRO}\\
        \cmidrule{1-6} \cmidrule{8-9}
        \multirow{5}{*}{{CNN/Daily Mail}} & GPT2  & -0.168 & -0.198 & -0.036 & -0.158 && -0.325(-0.091) & \toponehl{-0.510} (-0.227)  \\
        %\multirow{4}{*}{{CNN/Daily Mail}} & GPT2  & -0.168 & \topthreehl{-0.198} & -0.036 & -0.158 && -0.325 (-0.091) & \toponehl{-0.510} (-0.189) \\
        & LLaMA & -0.225 & \topthreehl{-0.420} & -0.086 & -0.415  && -0.380(-0.229) & \toponehl{-0.520}(-0.337)  \\
        & LLaMA2 & -0.096 & -0.109 &-0.139 & -0.110  && -0.370(-0.260) & \toponehl{-0.534}(-0.294)  \\
        & GPT3 & \toptwohl{-0.231} & -0.202 & -0.145 & -0.170 && \topthreehl{-0.229}(-0.100) & \toponehl{-0.394}(-0.244)  \\
        & GPT3.5 & -0.119 & -0.119 & -0.036 & -0.106 && \toponehl{-0.223}(-0.131) &\toptwohl{-0.220}(-0.158)	 \\
        \cellcolor{lightgray}& \cellcolor{lightgray}GPT2 & \cellcolor{lightgray}-0.021 & \cellcolor{lightgray}0.021 & \cellcolor{lightgray}-0.077 & \cellcolor{lightgray}0.014 && \cellcolor{lightgray}-0.333(-0.168) & \cellcolor{lightgray}\toponehl{-0.567} (-0.335) \\
        %\cellcolor{lightgray}& \cellcolor{lightgray}GPT2 & \cellcolor{lightgray}-0.0208 & \cellcolor{lightgray}\topthreehl{0.0212} & \cellcolor{lightgray}-0.077 & \cellcolor{lightgray}0.014 && \cellcolor{lightgray}-0.333 (-0.168) & \cellcolor{lightgray}\toponehl{-0.567} (-0.335) \\
        
        \cellcolor{lightgray}& \cellcolor{lightgray}LLaMA & \cellcolor{lightgray}0.025 & \cellcolor{lightgray}0.030 &
        \cellcolor{lightgray}\topthreehl{-0.040} & \cellcolor{lightgray}0.007 && \cellcolor{lightgray}-0.257 (-0.136) & \cellcolor{lightgray}\toponehl{-0.655} (-0.396)  \\
        
 
        \cellcolor{lightgray}& \cellcolor{lightgray}LLaMA2 & \cellcolor{lightgray}-0.000 & \cellcolor{lightgray}-0.008&
        \cellcolor{lightgray}0.008 & \cellcolor{lightgray} -0.018 && \cellcolor{lightgray}-0.196(-0.006) & \cellcolor{lightgray}\toponehl{-0.300}(0.024)  \\
        
        
        \cellcolor{lightgray}& \cellcolor{lightgray}GPT3 & \cellcolor{lightgray}-0.054 & \cellcolor{lightgray}-0.207 & \cellcolor{lightgray}-0.016 & \cellcolor{lightgray}-0.172 && \cellcolor{lightgray}\topthreehl{-0.236}(-0.084) & \cellcolor{lightgray}\toponehl{-0.382}(-0.140)	  \\
        \multirow{-5}{*}{\cellcolor{lightgray}{Eli5-Category}}& \cellcolor{lightgray}GPT3.5 & \cellcolor{lightgray}-0.037 & \cellcolor{lightgray}\toptwohl{-0.240} & \cellcolor{lightgray}-0.084 & \cellcolor{lightgray}\toponehl{-0.289} && \cellcolor{lightgray}-0.168(-0.021) & \cellcolor{lightgray}\topthreehl{-0.223}(-0.046)  \\
        \multirow{5}{*}{{Wiki-QA}} & GPT2 & -0.110 & -0.003 & -0.134 & -0.004 && -0.433(-0.150) & \toponehl{-0.682} (-0.434)  \\
        %\multirow{4}{*}{{Wiki-QA}} & GPT2 & -0.110 & -0.003 & \topthreehl{-0.134} & -0.004 && -0.433 (-0.150) & \toponehl{-0.682} (-0.434) \\

        & LLaMA & -0.057 & 0.033 & -0.099 & -0.020 && -0.347(-0.260)	 & \toponehl{-0.598}(-0.468)	 \\
        & LLaMA2 & -0.181 & \topthreehl{-0.193} & -0.166 & -0.140 && \toptwohl{-0.281}(-0.206) & \toponehl{-0.374}(-0.184)	 \\
        
        & GPT3 & -0.112 & -0.192 & 0.017 & -0.107 && \toptwohl{-0.326}(-0.061) & \toponehl{-0.376}(-0.139)  \\
        & GPT3.5 & -0.051 & -0.107 & -0.065 & -0.105 && \toptwohl{-0.401}(-0.085) & \toponehl{-0.425}(-0.079) \\
        \cellcolor{lightgray}&  \cellcolor{lightgray}GPT2& \cellcolor{lightgray}0.239 & \cellcolor{lightgray}0.073 & \cellcolor{lightgray}\topthreehl{0.282} & \cellcolor{lightgray}0.081 && \cellcolor{lightgray}\toptwohl{-0.556} (-0.253) & \cellcolor{lightgray}\toponehl{-0.656} (-0.276)  \\
        \cellcolor{lightgray}& \cellcolor{lightgray}LLaMA & \cellcolor{lightgray}-0.044 & \cellcolor{lightgray}-0.153 & \cellcolor{lightgray}-0.060 & \cellcolor{lightgray}\topthreehl{-0.166} && \cellcolor{lightgray}\toptwohl{-0.472} (-0.353) & \cellcolor{lightgray}\toponehl{-0.837} (-0.636)  \\

        
        \cellcolor{lightgray}& \cellcolor{lightgray}LLaMA2 & \cellcolor{lightgray}0.157 & \cellcolor{lightgray}-0.000 & \cellcolor{lightgray}\toptwohl{0.185} & \cellcolor{lightgray}-0.015 && \cellcolor{lightgray}0.068(0.009) & \cellcolor{lightgray}0.125(\topthreehl{0.163})  \\
        
        \cellcolor{lightgray}& \cellcolor{lightgray}GPT3 & \cellcolor{lightgray}-0.046 & \cellcolor{lightgray}-0.162 & \cellcolor{lightgray}-0.039 & \cellcolor{lightgray} -0.176 && \cellcolor{lightgray}-0.250(\toptwohl{-0.254}) & \cellcolor{lightgray}-0.251(\toponehl{-0.339})  \\
        \multirow{-5}{*}{\cellcolor{lightgray}{WMT 2014}} & \cellcolor{lightgray}GPT3.5 & \cellcolor{lightgray}0.089 & \cellcolor{lightgray}-0.158 & \cellcolor{lightgray}0.050 & \cellcolor{lightgray}\topthreehl{-0.175} && \cellcolor{lightgray}\toptwohl{-0.244}(-0.065) & \cellcolor{lightgray}\topthreehl{-0.233}(-0.017)  \\
        \bottomrule
        \end{tabular}
        }
  \end{subtable}
  \vspace{1mm}
  \vfill
  \begin{subtable}[h]{\textwidth}
  \setlength{\tabcolsep}{10.13pt}
  \centering
  %\responseref{}
  % \caption{Perturbation-based Uncertainty Estimation}
  \scriptsize
  \resizebox{0.95\linewidth}{!}{
    \begin{tabular}{llcccccc}
        \toprule
        \multirow{2}{*}{\textbf{Dataset}}&\multirow{2}{*}{\textbf{LLM}} & \multicolumn{6}{c}{\textbf{Perturbation-based}}\\
        \cmidrule{3-8}
        && \textbf{Max VR} & \textbf{Max VRO} & \textbf{Min VR} & \textbf{Min VRO} & \textbf{MaxDiff VR} & \textbf{MaxDiff VRO} \\
        \midrule
        
        \multirow{5}{*}{CNN/Daily Mail} & GPT2 & 0.407 (\toptwohl{0.448}) & 0.356(0.430) & 0.260(0.269) & 0.376(0.403) & 0.400(\topthreehl{0.436}) & 0.397(0.439) \\

        
        & LLaMA & 0.447(\toptwohl{0.504}) & 0.410(0.484) & 0.324(0.335) & 0.443(\topthreehl{0.495}) & 0.420(0.469) & 0.429(0.479)  \\
        & LLaMA2 &  -0.204(-0.161) & \topthreehl{-0.388}(-0.154) & -0.075(-0.055) & \toptwohl{-0.418}(-0.226) & -0.194(-0.152) & -0.378(-0.143)  \\
       
        & GPT3 &  -0.096(-0.084) & -0.233(-0.209) & -0.001(-0.049) & 0.034(0.041) & -0.119(-0.121) & -0.228(-0.182)	  \\
        -	
        & GPT3.5 & 0.064(-0.086) & -0.024(-0.087) & -0.116(-0.176) & -0.068(\topthreehl{-0.177}) & -0.042(-0.138) & 0.072(0.021)  \\
        
        \cellcolor{lightgray} & \cellcolor{lightgray}GPT2 & \cellcolor{lightgray}-0.251(-0.158) & \cellcolor{lightgray}\topthreehl{-0.414}(-0.247) & \cellcolor{lightgray}-0.055(-0.081) & \cellcolor{lightgray}-0.121(-0.186) & \cellcolor{lightgray}-0.268(-0.174) & \cellcolor{lightgray}\toptwohl{-0.473}(-0.284)		 \\

        \cellcolor{lightgray} & \cellcolor{lightgray}LLaMA & \cellcolor{lightgray}-0.163(-0.100) & \cellcolor{lightgray}\toptwohl{-0.442}(-0.258) & \cellcolor{lightgray}-0.143(-0.140) & \cellcolor{lightgray}-0.102(-0.142) & \cellcolor{lightgray}-0.172(-0.073) & \cellcolor{lightgray}\topthreehl{-0.357}(-0.178)  \\


        \cellcolor{lightgray} & \cellcolor{lightgray}LLaMA2 & \cellcolor{lightgray}-0.079(0.008) & \cellcolor{lightgray}-0.203(-0.017) & \cellcolor{lightgray}-0.086(0.002) & \cellcolor{lightgray}\toptwohl{-0.218}(0.026) & \cellcolor{lightgray}-0.086(0.018) & \cellcolor{lightgray}\topthreehl{-0.210}(-0.011)	  \\
        
        \cellcolor{lightgray} & \cellcolor{lightgray}GPT3 & \cellcolor{lightgray}0.168(0.179) & \cellcolor{lightgray}0.026(0.079) & \cellcolor{lightgray}\toptwohl{-0.236}(-0.246) & \cellcolor{lightgray}-0.066(-0.135) & \cellcolor{lightgray} 0.140(-0.003) & \cellcolor{lightgray}0.184(0.047) \\

        % 0.003(-0.076)	0.065(0.049)	-0.087(-0.157)	0.072(0.056)	0.160(0.092)	0.183(0.125)	
        \multirow{-5}{*}{\cellcolor{lightgray}{Eli5-Category}} & \cellcolor{lightgray}GPT3.5 & \cellcolor{lightgray}0.003(-0.076) & \cellcolor{lightgray}0.065(0.049) & \cellcolor{lightgray}-0.087(-0.157) & \cellcolor{lightgray}0.072(0.056) & \cellcolor{lightgray}0.160(0.092) & \cellcolor{lightgray}0.183(0.125)\\
        \multirow{5}{*}{Wiki-QA} & GPT2 & \topthreehl{-0.441}(-0.284) &\toptwohl{-0.617}(-0.373) & -0.169(-0.186) &-0.136(-0.145) & -0.270(-0.107) & -0.557(-0.279)	 \\
        & LLaMA & -0.200(-0.126) & \toptwohl{-0.478}(-0.416) & -0.090(-0.206) & -0.135(-0.348) & -0.227(-0.257) & -0.338(\topthreehl{-0.404}) \\
        & LLaMA2 & -0.057(0.050) & -0.081(0.014) & -0.064(-0.001) & -0.164(-0.036) & -0.077(0.023) & -0.111(-0.006) \\
	
        & GPT3 & -0.064(0.049) & -0.204(-0.186) & -0.042(0.048) & \topthreehl{-0.247}(-0.146) & -0.042(-0.020) & -0.095(-0.111)	 \\
        & GPT3.5 & 0.092(0.065) & 0.078(0.056) & -0.017(-0.113) & -0.030(-0.109) & 0.157(0.014) & \topthreehl{0.214}(0.065) \\
        \cellcolor{lightgray} & \cellcolor{lightgray}GPT2 & \cellcolor{lightgray} -0.025(0.067) & \cellcolor{lightgray}0.042(0.071) & \cellcolor{lightgray}-0.059(0.009) & \cellcolor{lightgray}0.020(0.077) & \cellcolor{lightgray}-0.093(-0.010) & \cellcolor{lightgray}-0.041(0.007)	  \\

        \cellcolor{lightgray} & \cellcolor{lightgray}LLaMA & \cellcolor{lightgray}0.153(0.086) & \cellcolor{lightgray}0.099(-0.153) & \cellcolor{lightgray}0.094(0.055) & \cellcolor{lightgray}0.155(0.009) & \cellcolor{lightgray}-0.038(-0.033) & \cellcolor{lightgray}-0.012(-0.150)	 \\

        % -0.022(-0.027)	-0.036(0.058)	-0.064(-0.029)	-0.190(0.024)	-0.026(-0.028)	-0.040(0.058)	
        
        \cellcolor{lightgray} & \cellcolor{lightgray}LLaMA2 & \cellcolor{lightgray}-0.022(-0.027)) & \cellcolor{lightgray}-0.036(0.058) & \cellcolor{lightgray}-0.064(-0.029) & \cellcolor{lightgray}\toponehl{-0.190}(0.024) & \cellcolor{lightgray}-0.026(-0.028) & \cellcolor{lightgray}-0.040(0.058)	 \\

        
        \cellcolor{lightgray} & \cellcolor{lightgray}GPT3 & \cellcolor{lightgray}-0.076(0.006) & \cellcolor{lightgray}0.016(0.021) & \cellcolor{lightgray}-0.033(0.095) & \cellcolor{lightgray}\topthreehl{0.215}(0.138) & \cellcolor{lightgray}-0.103(0.001) & \cellcolor{lightgray}0.013(0.040)  \\
        \multirow{-5}{*}{\cellcolor{lightgray}WMT 2014} & \cellcolor{lightgray}GPT3.5 & \cellcolor{lightgray} -0.277(\toponehl{-0.363}) & \cellcolor{lightgray}-0.101(-0.081) & \cellcolor{lightgray}-0.099(-0.048) & \cellcolor{lightgray}-0.007(-0.003)  & \cellcolor{lightgray}-0.105(-0.201) & \cellcolor{lightgray}-0.031(-0.024)  \\
        \bottomrule
    \end{tabular}
    }
    \end{subtable}
    % \vspace{-10pt}
    
\label{tab:evaluation_corrNLP}
\end{table*}
\fi


\begin{table*}[htbp]
  \centering
  \caption{Correlation between uncertainty scores and models' performance on NLP tasks. Values presented prior to the bracket represent the uncertainty scores are computed based on cosine score between embeddings. Conversely, values in the bracket represent scores computed via task-specific distance functions.}
  \begin{minipage}{0.45\textwidth}
    \centering
    \caption*{(a) Single-inference Uncertainty Estimation}
    \scriptsize
        \begin{tabular}{lcccc}
        \toprule
        \textbf{Model / Dataset} & \textbf{Max Prob} & \textbf{Average Prob} & \textbf{Max Ent} & \textbf{Average Ent} \\
        \midrule
        GPT2 (CNN Daily) & -0.168 & \hl{-0.198} & -0.036 & -0.158 \\
        LLAMA (CNN Daily) & -0.225 & \hl{-0.420} & -0.086 & -0.415 \\
        GPT3 (CNN Daily) & \hl{-0.231} & -0.202 & -0.145 & -0.170 \\
        GPT3.5 (CNN Daily) & \hl{-0.1187} & -0.1186 & -0.036 & -0.106 \\
        \cellcolor{lightgray}GPT2 (Eli5 Category) & \cellcolor{lightgray}-0.0208 & \cellcolor{lightgray}\hl{0.0212} & \cellcolor{lightgray}-0.077 & \cellcolor{lightgray}0.014 \\
        
        \cellcolor{lightgray}LLAMA (Eli5 Category) & \cellcolor{lightgray}0.025 & \cellcolor{lightgray}0.030 & \cellcolor{lightgray}\hl{-0.040} & \cellcolor{lightgray}0.007 \\
        
        \cellcolor{lightgray}GPT3 (Eli5 Category) & \cellcolor{lightgray}-0.054 & \cellcolor{lightgray}\hl{-0.207} & \cellcolor{lightgray}-0.016 & \cellcolor{lightgray}-0.172 \\
        
        \cellcolor{lightgray}GPT3.5 (Eli5 Category) & \cellcolor{lightgray}-0.037 & \cellcolor{lightgray}-0.240 & \cellcolor{lightgray}-0.084 & \cellcolor{lightgray}\hl{-0.289} \\
        GPT2 (WIKI) & -0.110 & -0.003 & \hl{-0.134} & -0.004 \\
        LLAMA (WIKI) & -0.057 & 0.033 & -0.099 & -0.020 \\
        GPT3 (WIKI) & -0.112 & \hl{-0.192} & 0.017 & -0.107 \\
        GPT3.5 (WIKI) & -0.051 & \hl{-0.107} & -0.065 & -0.105 \\
        \cellcolor{lightgray}GPT2 (WMT14) & \cellcolor{lightgray}\hl{0.239} & \cellcolor{lightgray}0.073 & \cellcolor{lightgray}0.282 & \cellcolor{lightgray}0.081 \\
        \cellcolor{lightgray}LLAMA (WMT14) & \cellcolor{lightgray}-0.044 & \cellcolor{lightgray}-0.153 & \cellcolor{lightgray}-0.060 & \cellcolor{lightgray}\hl{-0.166} \\
        \cellcolor{lightgray}GPT3 (WMT14) & \cellcolor{lightgray}-0.046 & \cellcolor{lightgray}-0.162 & \cellcolor{lightgray}-0.039 & \cellcolor{lightgray}\hl{-0.176} \\
        \cellcolor{lightgray}GPT3.5 (WMT14) & \cellcolor{lightgray}0.089 & \cellcolor{lightgray}-0.158 & \cellcolor{lightgray}0.050 & \cellcolor{lightgray}\hl{-0.175} \\
        \bottomrule
        \end{tabular}
  \end{minipage}\hfill
  \begin{minipage}{0.45\textwidth}
    \centering
    \caption*{(b) Sample-based Uncertainty Estimation}
    \scriptsize
        \begin{tabular}{lcc}
            \toprule
            \textbf{Model / Dataset} & \textbf{Sample VR} & \textbf{Sample VRO} \\
            \midrule
            GPT2 (CNN Daily) & -0.325(-0.091) & \hl{-0.510}(-0.189) \\
            LLAMA (CNN Daily) & -0.380(-0.236) & \hl{-0.520}(-0.324) \\
            GPT3 (CNN Daily) & -0.326(-0.210) & \hl{-0.413}(-0.268) \\
            GPT3.5 (CNN Daily) & -0.288(-0.181) & \hl{-0.295}(-0.191) \\
            \cellcolor{lightgray}GPT2 (Eli5 Category) & \cellcolor{lightgray}-0.333(-0.168) & \cellcolor{lightgray}\hl{-0.567}(-0.335) \\
            \cellcolor{lightgray}LLAMA (Eli5 Category) & \cellcolor{lightgray}-0.257(-0.136) & \cellcolor{lightgray}\hl{-0.655}(-0.396) \\
            \cellcolor{lightgray}GPT3 (Eli5 Category) & \cellcolor{lightgray}-0.275(-0.136) & \cellcolor{lightgray}\hl{-0.359}(-0.164) \\
            \cellcolor{lightgray}GPT3.5 (Eli5 Category) & \cellcolor{lightgray}-0.224(-0.053) & \cellcolor{lightgray}\hl{-0.253}(-0.061) \\
            GPT2 (WIKI) & -0.433(-0.150) & \hl{-0.682}(-0.434) \\
            LLAMA (WIKI) & -0.347(-0.260) & \hl{-0.598}(-0.468) \\
            GPT3 (WIKI) & -0.435(-0.151) & \hl{-0.449}(-0.164) \\
            GPT3.5 (WIKI) & -0.341(-0.077) & \hl{-0.380}(-0.080) \\
            \cellcolor{lightgray}GPT2 (WMT14) & \cellcolor{lightgray}-0.556(-0.253) & \cellcolor{lightgray}\hl{-0.656}(-0.276) \\
            \cellcolor{lightgray}LLAMA (WMT14) & \cellcolor{lightgray}-0.472(-0.353) & \cellcolor{lightgray}\hl{-0.837}(-0.636)\\
            \cellcolor{lightgray}GPT3 (WMT14) & \cellcolor{lightgray}-0.228(-0.275) & \cellcolor{lightgray}-0.235(\hl{-0.306}) \\
            \cellcolor{lightgray}GPT3.5 (WMT14) & \cellcolor{lightgray}-0.272(-0.075) & \cellcolor{lightgray}\hl{-0.282}(-0.045) \\
            \bottomrule
        \end{tabular}
  \end{minipage}
  \vfill
  \centering
  \caption*{(c) Perturbation-based Uncertainty Estimation}
  \scriptsize
    \begin{tabular}{lcccccc}
        \toprule
        \textbf{Model / Dataset} & \textbf{Max VR} & \textbf{Max VRO} & \textbf{Min VR} & \textbf{Min VRO} & \textbf{MaxDiff VR} & \textbf{MaxDiff VRO} \\
        \midrule
        GPT2 (CNN Daily) & 0.263(\hl{0.389}) & 0.143(0.350) & -0.039(0.254) & -0.239(0.292) & 0.065(0.339) & -0.227(0.289) \\
        
        LLAMA (CNN Daily) & 0.293(\hl{0.444}) & 0.118(0.403) & -0.025(0.329) & -0.315(0.277) & 0.036(0.362) & -0.325(0.294) \\

        GPT3 (CNN Daily) & -0.232(-0.166) & \hl{-0.34}(-0.216) & -0.100(-0.106) & -0.041(-0.045) & -0.296(-0.143) & -0.328(-0.159) \\
        GPT3.5 (CNN Daily) & -0.143(-0.029) & -0.148(-0.015) & -0.065(-0.102) & -0.084(-0.118) & \hl{-0.316}(-0.22) & -0.283(-0.207) \\
        
        \cellcolor{lightgray}GPT2 (Eli5 Category) & \cellcolor{lightgray}-0.453(-0.173) & \cellcolor{lightgray}-0.456(-0.182) & \cellcolor{lightgray}-0.243(-0.107) & \cellcolor{lightgray}-0.241(-0.13) & \cellcolor{lightgray}\hl{-0.471}(-0.165) & \cellcolor{lightgray}-0.47(-0.179) \\
        
        \cellcolor{lightgray}LLAMA (Eli5 Category) & \cellcolor{lightgray}-0.562(-0.181) & \cellcolor{lightgray}\hl{-0.565}(-0.196) & \cellcolor{lightgray}-0.406(-0.150) & \cellcolor{lightgray}-0.434(-0.160) & \cellcolor{lightgray}-0.541(-0.168) & \cellcolor{lightgray}-0.537(-0.181) \\
        
        \cellcolor{lightgray}GPT3 (Eli5 Category) & \cellcolor{lightgray}-0.085(0.128) & \cellcolor{lightgray}-0.112(0.106) & \cellcolor{lightgray}-0.108(-0.010) & \cellcolor{lightgray}-0.118(-0.007) & \cellcolor{lightgray}-0.071(-0.117) & \cellcolor{lightgray}\hl{-0.15}(-0.143) \\
        
        \cellcolor{lightgray}GPT3.5 (Eli5 Category) & \cellcolor{lightgray}-0.033(-0.042) & \cellcolor{lightgray}-0.050(-0.034) & \cellcolor{lightgray}-0.005(-0.067) & \cellcolor{lightgray}0.021(-0.031) & \cellcolor{lightgray}-0.111(-0.134) & \cellcolor{lightgray}\hl{-0.118}(-0.110) \\
        
        GPT2 (WIKI) & -0.599(-0.132) & -0.577(-0.139) & -0.433(-0.152) & -0.426(-0.140) & \hl{-0.617}(-0.138) & -0.607(-0.149) \\
        
        LLAMA (WIKI) & -0.379(-0.193) & -0.428(-0.214) & -0.385(-0.190) & -0.432(-0.208) & -0.507(-0.227) & \hl{-0.527}(-0.239) \\
        GPT3 (WIKI) & -0.173(-0.132) & -0.291(-0.290) & -0.074(-0.063) & -0.149(-0.182) & -0.338(-0.255) & \hl{-0.457}(-0.378) \\
        GPT3.5 (WIKI) & \hl{-0.353}(-0.114) & -0.309(-0.110) & 0.082(-0.028) & 0.100(-0.047) & -0.345(-0.285) & -0.328(-0.277) \\
        
        \cellcolor{lightgray}GPT2 (WMT14) & \cellcolor{lightgray}-0.231(-0.005) & \cellcolor{lightgray}\hl{-0.24}(-0.133) & \cellcolor{lightgray}-0.072(-0.026) & \cellcolor{lightgray}-0.019(-0.129) & \cellcolor{lightgray}-0.226(-0.051) & \cellcolor{lightgray}-0.197(-0.101) \\
        
        \cellcolor{lightgray}LLAMA (WMT14) & \cellcolor{lightgray}-0.415(-0.285) & \cellcolor{lightgray}\hl{-0.417}(-0.307) & \cellcolor{lightgray}-0.208(0.033) & \cellcolor{lightgray}-0.195(0.140) & \cellcolor{lightgray}-0.349(-0.168) & \cellcolor{lightgray}-0.361(-0.118) \\
        
        \cellcolor{lightgray}GPT3 (WMT14) & \cellcolor{lightgray}-0.166(-0.073) & \cellcolor{lightgray}-0.169(-0.097) & \cellcolor{lightgray}-0.071(-0.133) & \cellcolor{lightgray}-0.077(-0.130) & \cellcolor{lightgray}-0.22(-0.094) & \cellcolor{lightgray}\hl{-0.252}(-0.114) \\
        \cellcolor{lightgray}GPT3.5 (WMT14) & \cellcolor{lightgray}\hl{-0.476}(-0.466) & \cellcolor{lightgray}-0.475(-0.442) & \cellcolor{lightgray}-0.231(-0.278) & \cellcolor{lightgray}-0.194(-0.255) & \cellcolor{lightgray}-0.464(-0.355) & \cellcolor{lightgray}-0.439(-0.349) \\
        \bottomrule
    \end{tabular}
    \label{tab:evaluation_corrNLP}
\end{table*}
